The Star Height Hierarchy Vs. The Variable Hierarchy

The star height hierarchy (resp. the variable hierarchy) results in classifying $\mu$-terms into classes according to the nested depth of fixed point operators (resp. to the number of bound variables). We prove, under some assumptions, that the variable hierarchy is a proper refinement of the star height hierarchy. We mean that the non collapse of the variable hierarchy implies the non collapse of the star height hierarchy. The proof relies on the combinatorial characterization of the two hierarchies.

==> macros.tex <==
%% PACKAGES
\RequirePackage{comment}
\RequirePackage{ifthen}

\newcommand{\myqed}{}
\newcommand{\cutout}[1]{}
\newcommand{\longversion}[1]{}
%% WORKING VERSION
\def\workingversion{}
\ifthenelse{\isundefined{\workingversion}}%
{%
\excludecomment{workingversion}
\includecomment{cleanversion}
}
{
\includecomment{workingversion}
\excludecomment{cleanversion}
}


\newenvironment{keywords}{\textbf{Key words.}}{}

\begin{workingversion}
  \newenvironment{tbs}{%
    \renewcommand{\labelitemi}{$\blacktriangleright$}%
    \begin{itemize}\tt }{\end{itemize}}
  %%
  \newcommand{\shtbs}[1]{\begin{tbs} \item #1 \end{tbs}}
  %%
  \newcommand{\tobesaid}[1]{\shtbs{#1}}
  %%
\end{workingversion}

\begin{cleanversion}
  \newcommand{\tobesaid}[1]{}
\end{cleanversion}

%% SPACES
\newcommand{\myhspace}[1]{\mbox{\hspace{#1}}}

%% ENVIRONMENTS
%%\itemsep=0mm
% \newenvironment{myitemize}[1][$\bullet$]{%
%   \begin{list}{#1}{%
%       \leftmargin=2.2mm%
%       \labelsep=1mm%
%       \itemsep=0mm%
%       \labelwidth=1mm%
%       \parsep=1mm
% }%
% }{\end{list}}

\newenvironment{myitemize}[1][$\bullet$]
{\begin{itemize}}{\end{itemize}}

\newenvironment{myenumerate}{%
  \setcounter{enumi}{0}
  \begin{list}{\theenumi}{%
      \leftmargin=2.2mm%
      \labelsep=1mm%
      \itemsep=0mm%
      \labelwidth=1mm%
      \parsep=1mm
}%
}{\stepcounter{enumi}\end{list}}

%%
\newcommand{\mymod}{\,\mathrm{mod}\,}
\newcommand{\hier}[1]{\mathcal{L}(#1)}
\newcommand{\card}[1]{|#1|}
\newcommand{\sh}[1]{{\cal{H}}(#1)}
\newcommand{\monespace}[1]{\textrm{ }\hspace{#1}}
\newcommand{\Ent}[1]{\mathscr{E}(#1)}
\newcommand{\Entv}[1]{\mathscr{E}^{V}(#1)}
\newcommand{\gr}{{\varrho}}
\newcommand{\ver}[1]{{#1}^{v}}
\newcommand{\on}[1]{\overline{#1}}
\newcommand{\z}{{4n}}
\newcommand{\grnk}[1]{{\mathscr{R}^{B}}(#1)}
\newcommand{\Grnk}[1]{\mathscr{R}(#1)}
\newcommand{\spec}[1]{\partial{#1}}
\newcommand{\minus}[1]{{#1}^{-}}
\newcommand{\LD}{\mathscr{L}_4}
\newcommand{\CD}{\mathscr{C}_2}
\newcommand{\RD}{\mathscr{R}_4}
\newcommand{\scc}[1]{SCC(#1)}
\newcommand{\rnk}[1]{r(#1)}
\newcommand{\class}[1]{\mathscr{C}(#1)}
\newcommand{\classe}{\mathscr{C}}
\newcommand{\exclud}{\mathscr{F}}
\newcommand{\latt}[1]{\mathfrak{#1}}
\newcommand{\Boolmu}{\mathbb{L}_{\mu}}
\newcommand{\Lmu}{\mathbb{L}_{\mu}}
\newcommand{\mucalc}{\mathcal{T}_{\mu}}
\newcommand{\gameof}[1]{\gamma(#1)}
\newcommand{\graphof}[1]{\overline{#1}}
\newcommand{\sub}{\backslash}
\newcommand{\Comp}[1]{\mathbb{C}(#1)}
\newcommand{\termof}[1]{\tau(#1)}

\newcommand{\G}{{\cal G}}
\newcommand{\Gv}{\G^{\vec{}}}
\newcommand{\LG}{\mathcal{L}}


\newcommand{\sw}{$\star_w$}

\newcommand{\Med}[1]{\homl {#1} \homr}
\newcommand{\Seq}[2]{{#1}  \vdash {#2}}
\newcommand{\Str}[1]{{\mathscr {P}}(#1)}
\newcommand{\StrP}[2]{{{\mathscr{P}}_{#1}}(#2)}
\newcommand{\ET}[1]{\widetilde{{\mathscr{E}}}(#1)}
\newcommand{\ETT}[1]{\widehat{{\cal E}}(#1)}
\newcommand{\HT}[1]{\widehat{#1}}
\newcommand{\CH}[1]{{\mathscr{A}}_{#1}}
\newcommand{\WT}[1]{\widetilde{#1}}
\newcommand{\BL}[1]{{#1}_{\bullet}}
\newcommand{\BBL}[1]{{#1}_{\bullet \bullet}}
\newcommand{\Type} {\mathbb{T}}
\newcommand{\Pip}{\Pi^{+}}
\newcommand{\bridge}[1]{[{#1}]}

\newcommand{\rTo}{\longrightarrow}

\newcommand{\set}[1]{\{\,#1\,\}}
\newcommand{\couple}[1]{#1}
\newcommand{\collapserename}{1\textrm{-Sum}}

\newcommand{\id}{\mathtt{id}} 

\newcommand{\tiff}{\text{ iff }}
 \newcommand{\tif}{\text{ if }}
 \newcommand{\tand}{\text{ and }}
 \newcommand{\timplies}{\text{ implies }}
 \newcommand{\tor}{\text{ or }}
 \newcommand{\tst}{\text{ s.t. }}
 \newcommand{\twith}{\text{ with }}

\newlength{\myhidel}
\newcommand{\myhide}[1]{%
  \settowidth{\myhidel}{$#1$}%
  \mbox{\hspace{\myhidel}}%
}

\newcounter{casecounter}
\def\thecasecounter{(\roman{casecounter})}
\newenvironment{proofbycases}[1][0]{
  \setcounter{casecounter}{#1}%
}{}

\newenvironment{caseinproof}{%
  \refstepcounter{casecounter}%
  %\ifthenelse{\equal{casecounter}{1}}{}{\par}%
  \vskip 1pt
  \noindent%
  \emph{Case~\thecasecounter.}~
}{\par}

\newcommand{\acompleter}{\par\ldots A COMPLETER \ldots \par}
\newcommand{\acompleterdici}{\par\ldots A COMPLETER D'ICI\ldots \par}
\newcommand{\EXERCICEPOURWALID}{\par\ldots EXERCICE POUR WALID \ldots
  \par}

%% CORRECTIONS 

\newcommand{\acomment}[2]{$-\!\!\!\!>$ \emph{#1} $<\!\!\!\!-$\footnote{#2}}
\newcommand{\luigi}{\emph{Luigi suggestion}:~ }


%% SECTIONING
\newcommand{\breath}{\vskip 6pt}
\newcommand{\myparagraph}[1]{\breath\par\noindent\textbf{#1}~}



\renewcommand{\lefteqn}[2][0mm]{\makebox[#1][l]{$#2$}}


%\newcommand{\card}{\mathrm{card}\,}
%\newcommand{\dom}{\mathrm{dom}\,}
%\newcommand{\cod}{\mathrm{cod}\,}
\newcommand{\desc}[1]{\overline{#1}}
\newcommand{\eql}{\bigl [}
\newcommand{\eqr}{\bigr ]}
\newcommand{\myemph}[1]{\emph{#1}}
% \newcommand{\homl}{\bigl \langle}
% \newcommand{\homr}{\bigr \rangle}
\newcommand{\homl}{\langle}
\newcommand{\homr}{\rangle}
\newcommand{\meet}{\wedge}
\newcommand{\bigmeet}{\bigwedge}
\newcommand{\join}{\vee}
\newcommand{\bigjoin}{\bigvee}
 \newcommand{\Sup}{\textrm{\textbf{sup }}}
 \newcommand{\Inf}{\textrm{\textbf{inf }}}
\newcommand{\Mod}[1]{\mathrm{#1}}
\newcommand{\Theory}[1]{\mathbb{#1}}

%\newcommand{\mod}{\,\mathrm{mod}\,}
\renewcommand{\cong}{\equiv}
\newcommand{\reach}[1]{\overline{#1}}
\newcommand{\chain}{\sqsubset}
\newcommand{\schain}{\sqsubset_{\sigma}}
\newcommand{\pchain}{\sqsubset_{\pi}}
\newcommand{\comps}{||}
\newcommand{\compp}{\star}
\newcommand{\hide}{\backslash}
\newcommand{\TBE}{\mathcal{L}}
\newcommand{\Jprim}{\mathcal{K}}
\newcommand{\nnumbers}{\mathbb{N}}

%\newcommand{\Rho}{\Re}
\newcommand{\Rho}{\Upsilon}

\newcommand{\simulates}[1][]{\vartriangleright_{#1}}
\newcommand{\source}{\delta_{0}}
\newcommand{\target}{\delta_{1}}

%\renewcommand{\above}{\rightarrow^{*}}
\renewcommand{\above}{\text{ is an ancestor of }}
%\newcommand{\below}{\text{ is in the subtree of }}


%%%%%%%%%%%%%%%%%
%%% xypic
%%%%%%%%%%%%%%%%%


\newcommand{\myxygraph}[2][6em]{
  \mbox{$\begin{array}{@{\hspace{0mm}}c@{\hspace{0mm}}}
      \xy\xygraph{!{<#1,0cm>:<0cm,#1>::}#2}\endxy
    \end{array}$}
  }

%\def\deplacement{d(0.1)r(0.2)}
%\newgraphescape{p}[1]{[]*+{#1}([u(0.5)r(0.2)]*+{\pi})}

%\newgraphescape{p}[1]{[]*+{#1}*\cir{}="P"([d(0.2)r(0.4)]*+{\pi})}
\newgraphescape{p}[1]{[]*+{#1}*\cir{}="P"([d(0.2)r(0.4)]*+{\textrm{A}})}
%\newgraphescape{P}[1]{[]*++{#1}*\cir{}="P"([d(0.12)r(0.29)]*+{\pi})}
\newgraphescape{P}[1]{[]*++{#1}*\cir{}="P"([d(0.12)r(0.29)]*+{A})}


%\newgraphescape{s}[1]{[]*+{#1}*\cir{}="P"([d(0.2)r(0.4)]*+{\sigma})}
\newgraphescape{s}[1]{[]*+{#1}*\cir{}="P"([d(0.2)r(0.4)]*+{\textrm{E}})}
\newgraphescape{o}[1]{[]*+{#1}*\cir{}}
\newgraphescape{O}[1]{[]*++{#1}*\cir{}}

\newgraphescape{g}[1]{%
  []!s{v_{#1,1}}(:[l]!o{x_{#1,1}})
  :[d]!p{v_{#1,2}}(:[l]!o{x_{#1,2}})
  :[d]!s{v_{#1,3}}(:[l]!o{x_{#1,3}})
  :[d]!p{v_{#1,4}}(:[l]!o{x_{#1,4}})
  :[d]!s{v_{#1,5}}(:[l]!o{x_{#1,5}})
  "P"="E_{#1}"
}




\newgraphescape{a}[1]{[]*+{#1}*\frm{o}="P"([d(0.2)r(0.4)]*+{\pi})}
\newgraphescape{b}[1]{[]*+{#1}*\frm{o}="P"([d(0.2)r(0.4)]*+{\sigma})}
\newgraphescape{c}[1]{[]*+{#1}*\frm{o}}

\newgraphescape{j}[1]{%
  []!b{a_{#1,1}}(:[l]!c{x_{#1,1}})"P"="B_{#1}"
  :[d]!a{a_{#1,2}}(:[l]!c{x_{#1,2}})
  :[d]!b{a_{#1,3}}(:[l]!c{x_{#1,3}})
  :[d]!a{a_{#1,4}}(:[l]!c{x_{#1,4}})
  :[d]!b{a_{#1,5}}(:[l]!c{x_{#1,5}})
  "P"="E_{#1}"
}


%\newgraphescape{p}#1{[]*+[F]+[]{#1}} 
% \newgraphescape{p}#1{[]*=<1.6em>[o]{#1}*\frm{o}} 

% \newgraphescape{g}#1{
%   []="S"[d(0.05)]
%   ( -[d(0.6)d(0.6)l(0.6)]-[r(0.6)r(0.6)]-[r(0.6)l(0.6)],
%    -[d(0.6)d(0.6)r(0.6)]="RD")
%  [d(0.8)]*{#1}
% }

% \newgraphescape{G}#1{
%   []*{:}
%   [r(0.6)u(0.8)]
%   ( -[d(0.6)d(0.6)l(0.6)]-[r(0.6)r(0.6)]-[r(0.6)l(0.6)],
%    -[d(0.6)d(0.6)r(0.6)])
%  [d(0.8)]*{#1}
%  [r(0.6)]*{:}
% }


\newcommand\strategy[4][4]{
 \xy\xygraph{!{<#1pc,0pc>:<0pc,3pc>::} 
     []*{\firstplayer{#2}} [d]*{\secondplayer{#2}}
   #3
       }
   \endxy
 \hspace{10mm}
  \xy\xygraph{!{<#1pc,0pc>:<0pc,3pc>::} 
     #4
      }
  \endxy
  }

\newcommand\strategyw[4][4]{
 \xy\xygraph{!{<#1pc,0pc>:<0pc,3pc>::} 
     %[]*{\firstplayer{#2}} [d]*{\secondplayer{#2}}
   #3
       }
   \endxy
 \hspace{10mm}
  \xy\xygraph{!{<#1pc,0pc>:<0pc,3pc>::} 
     #4
      }
  \endxy
  }


% \newgraphescape{w}#1#2{
%   []!p{\firstplayer{#1}}="S" (:[r]!p{\firstvariable{#2}}) 
%   :[d]!p{\secondplayer{#1}} (:[r]!p{\secondvariable{#2}})
%   :[d]!p{\firstplayer{#1}} (:[r]!p{\thirdvariable{#2}}) 
%  }

% \newcommand{\firstvariable}[1]{\ifx#1a a_{0}\else b_{0}\fi}
% \newcommand{\secondvariable}[1]{\ifx#1a a_{1}\else b_{1}\fi}
% \newcommand{\thirdvariable}[1]{\ifx#1a a_{2}\else b_{2}\fi}
\newcommand{\firstvariable}[1]{\ifthenelse{\equal{#1}{a}}{a_{0}}{b_{0}}}
\newcommand{\secondvariable}[1]{\ifthenelse{\equal{#1}{a}}{a_{1}}{b_{1}}}
\newcommand{\thirdvariable}[1]{\ifthenelse{\equal{#1}{a}}{a_{2}}{b_{2}}}
\newcommand{\firstplayer}[1]{#1}
%\newcommand{\secondplayer}[1]{\ifx#1\pi\sigma \else \pi \fi}
\newcommand{\secondplayer}[1]{
  \ifthenelse{\equal{#1}{\pi}}{\sigma}{
    \ifthenelse{\equal{#1}{\sigma}}{\pi}{
      \ifthenelse{\equal{#1}{M}}{O}{M}
      }
    }
}

\ifx\TAC\undefined
\RequirePackage{ifthen}
\newcommand{\Whitstar}{}
\newcommand{\Whitvariablea}{a_{0}}
\newcommand{\Whitvariableb}{a_{1}}
\newcommand{\Whitvariablec}{a_{2}}
\newcommand{\Whitlabel}[3]{
  \ifthenelse{\equal{#2}{\pi}}{\renewcommand{\Whitstar}{}}
  {\renewcommand{\Whitstar}{*}}
  \ifthenelse{\equal{#3}{a}}{
   \renewcommand{\Whitvariablea}{a_{0}}
   \renewcommand{\Whitvariableb}{a_{1}}
   \renewcommand{\Whitvariablec}{a_{2}}
   }
  {\renewcommand{\Whitvariablea}{b_{0}}
   \renewcommand{\Whitvariableb}{b_{1}}
   \renewcommand{\Whitvariablec}{b_{2}}}
 W_{#1}^{\Whitstar}(\Whitvariablea,\Whitvariableb,\Whitvariablec)
}
\newgraphescape{A}#1#2#3#4#5{
  []!p{\firstplayer{#2}}="S"
  ( -[l(#4)]-[d(#5)]-[d(#5)]-[r(#4)]!p{\firstplayer{#2}}="B",
  -[r(#4)]-[d(#5)]-[d(#5)]-"B")
  [d(#5)]*{\Whitlabel{#1}{#2}{#3}}
  "B"
}
\newgraphescape{T}#1#2#3{[]!A{#1}{#2}{#3}{0.5}{0.8} }

% \newcommand{\mylabel}[1]{
%   \write\@auxout{\string
%     \newlabel{#1}{{\theenumi}{\thepage}}}
%     }
% \def\mylabel#1{\@bsphack\if@filesw {\let\thepage\relax
%    \xdef\@gtempa{\write\@auxout{\string
%       \newlabel{#1}{{\theenumi}{\thepage}}}}}\@gtempa
%    \if@nobreak \ifvmode\nobreak\fi\fi\fi\@esphack}
% \def\refcounter#1{\edef\@currentlabel{\csname p@#1\endcsname\csname the#1\endcsname}}
\fi


%%%%%%%%%%%%%%%%%%%%%%%
%%% Imported from FOSSACS03
\newcommand{\usubseteq}{\mathbin{\begin{rotate}{45}
        $\subseteq$\end{rotate}}}
\newcommand{\dsubseteq}{\mathbin{\begin{rotate}{-45}
        $\subseteq$\end{rotate}}}

\newcommand{\header}[1]{\par\noindent\textbf{#1}} %% header
\def\N{\mathbb{N}} %% natural numbers
%%def\set#1{\{#1\}} %% set former
%\newcommand{\rTo}{\longrightarrow} %% arrow to right.
\newcommand{\immprec}{\mapsto} %% out of component rel.
%\newcommand{\homl}{$\langle\!\langle$} %% left Mediator game delimiter
%\newcommand{\homr}{$\rangle\!\rangle$} %% right Mediator game delimiter
%\newcommand{\card}{\mathrm{card}\,} %% cardinality
\newcommand{\quotient}{\mbox{$/\hspace{-0.3em}\sim$}} %% quotient with \sim 
\newcommand{\Land}[1][]{{\textstyle\bigwedge_{#1}}} %% bigwedge
\newcommand{\Lor}[1][]{{\textstyle\bigvee_{\!\!#1\,}}} %% bogvee
\newcommand{\eval}[1]{|\!|#1|\!|} %% logical interpretation
\newcommand{\mscc}[1]{[\,#1\,]} %% maximal strongly connected component
%------------------------------
\renewcommand{\deg}[2][]{\mathrm{deg}_{#1}(#2)}


\newcommand{\Strat}{\mathcal{S}}


%% Graphs

\newcommand{\mystar}[2]{\varsigma^{#1}_{#2}}

\newcommand{\glue}{Gl}
\newcommand{\dead}{De}
\newcommand{\GLUING}{\Gamma}
\newcommand{\derived}{\partial}

\newcommand{\lcollapse}[2][]{\,\mbox{$\overline{\bigoplus}$}^{#1}_{#2}}
\newcommand{\collapse}[2][]{\,\mbox{$\bigoplus$}^{#1}_{#2}}

%% Complexity classes

\newcommand{\LOGSPACE}{\mathrm{LOGSPACE}}
\newcommand{\NLOGSPACE}{\mathrm{NLOGSPACE}}
\newcommand{\NP}{\mathrm{NP}}
\newcommand{\POL}{\mathrm{P}}
\newcommand{\EXP}{\mathrm{EXPTIME}}


%% Logics
\newcommand{\MLmu}{\mathbb{L}_{\mu}^{M}}
\newcommand{\K}{\mathbb{K}}
\newcommand{\FO}[1] {\textrm{FO}^{#1}}



%% Classes of graphs
\newcommand{\ETWO}{{\cal U}_{2}}
%\newcommand{\qed}{}
%---------------------------------------------------





%\newcommand{\Strat}{\mathcal{S}}
%\newcommand{\Ent}[1]{\mathcal{E}(#1)}
%\newcommand{\lcollapse}[2][]{\overline{\bigoplus}^{#1}_{#2}}

\newenvironment{myproof}[1]{\emph{Proof of #1.}}{\hspace{\stretch{1}}% 
                                                       \Box }



\renewcommand{\deg}[2][]{\mathrm{deg}_{#1}(#2)}

%% Graphs






%% Classes of graphs


%% Spaces


%  \newenvironment{abstract}{}{\emph{}}

\newcommand{\Ents}{\mathscr{E}}

%\newcommand{\rTo}{\longrightarrow}
%\newcommand{\tif}{\text{ if }}
%\newcommand{\tand}{\text{ and }}
%\newcommand{\ET}[1]{\widetilde{{\mathcal E}}(#1)}
\newcommand{\Cycl}[1]{{\mathscr{C}}(#1)}
%\newcommand{\cutout}[1]{}
%-------------------------------------------------



%added from Lyon
\newgraphescape{G}#1{
  []="L"[l(0.2)]
  [r(0.6)u(0.8)]
  ( -[d(0.6)d(0.6)l(0.6)]-[r(0.6)r(0.6)]-[r(0.6)l(0.6)],
   -[d(0.6)d(0.6)r(0.6)])
  [d(0.8)]*+{#1}="C"
%  [r(0.6)]*+{:}="R"
 [r(0.4)]="R"
}
%
\newgraphescape{c}{
  []="A0"
  [l(0.5)d(0.15)]*=<1em>[o][F]{}="A"
  [r]*=<1em>[o][F]{}="B"
  !{"A"!R}[d(0.0)]="AD"
  !{"B"!L}[d(0.0)]="BD"
  "AD"-@`{"A0"+(0,0.15)}"BD"
  "A0"
}
%
\newgraphescape{d}{
  []="A0"
  [u(0.5)r(0.15)]*=<1em>[o][F]{}="A"
  [d]*=<1em>[o][F]{}="B"
  !{"A"!D}[d(0.0)]="AD"
  !{"B"!U}[d(0.0)]="BD"
  "AD"-@`{"A0"+(-0.15,0)}"BD"
  "A0"
}
%
\newgraphescape{e}{
  []="A0"
  [u(0.5)l(0.15)]*=<1em>[o][F]{}="A"
  [d]*=<1em>[o][F]{}="B"
  !{"A"!D}[d(0.0)]="AD"
  !{"B"!U}[d(0.0)]="BD"
  "AD"-@`{"A0"+(0.15,0)}"BD"
  "A0"
}
%%
%attention
%\newgraphescape{p}[1]{
%  []*{#1}*+++[o]{}*+\frm{o}
%}

%
% \newgraphescape{E}[1]{
%   []!p{#1}="#1"
% }

\newgraphescape{E}[1]{
  []*{#1}*+++[o]{}*+\frm{o}="#1"
}
%---------

%%%% debut macro %%%%
\makeatletter
\renewcommand{\thefigure}{\ifnum \c@section>\z@ \thesection.\fi
 \@arabic\c@figure}
\@addtoreset{figure}{section}
\makeatother




%%%% fin macro %%%%

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "0"
%%% End: 


